FedSOL: Stabilized Orthogonal Learning with Proximal Restrictions in Federated Learning

Federated Learning (FL) aggregates locally trained models from individual clients to construct a global model. While FL enables learning a model with data privacy, it often suffers from significant performance degradation when clients have heterogeneous data distributions. This data heterogeneity causes the model to forget the global knowledge acquired from previously sampled clients after being trained on local datasets. Although the introduction of proximal objectives in local updates helps to preserve global knowledge, it can also hinder local learning by interfering with local objectives. To address this problem, we propose a novel method, Federated Stabilized Orthogonal Learning (FedSOL), which adopts an orthogonal learning strategy to balance the two conflicting objectives. FedSOL is designed to identify gradients of local objectives that are inherently orthogonal to directions affecting the proximal objective. Specifically, FedSOL targets parameter regions where learning on the local objective is minimally influenced by proximal weight perturbations. Our experiments demonstrate that FedSOL consistently achieves state-of-the-art performance across various scenarios.

==> rebuttal.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}
% \input{sec/rebuttal_header}

% \begin{document}
% \title{FedSOL: Stabilized Orthogonal Learning in Federated Learning}
% \maketitle
% \thispagestyle{empty}
% \appendix

% \paragraph{Overall Comments} 

% We are grateful for the valuable feedback from all reviewers. We emphasize that FedSOL is compatible with existing proximal objectives, effectively addresses the global-local knowledge trade-off in FL. Below, we've organized our responses by Reviewer Code (\textbf{\textcolor{orange!87!black}{fSbK}}, \textbf{\textcolor{orange!87!black}{3HiN}}, \textbf{\textcolor{orange!87!black}{K9F1}}) and corresponding Weaknesses (\textbf{W}).
% %We are grateful for the valuable feedback and suggestions from all reviewers.  We have addressed all concerns raised, but please understand that we could not include every detail due to the 1-page limit. 

% %Rebuttal Contents
% \vspace{-6pt}
% \paragraph{\textcolor{orange!87!black}{fSbK}\,-\,W1 (Performance on Larger Datasets)} In \textbf{Table 2}, we show that FedSOL consistently achieves performance gains, while most existing FL (Federated Learning) methods are sensitive to learning setups. Although FedNTD marginally outperforms FedSOL in some CIFAR-10 cases, it significantly falls behind in most others. In \autoref{tab:cifar100_imagenet100}, we conducted experiments on the CIFAR-100 and ImageNet-100 datasets. We used the ResNet-18 model, distributing each dataset across 100 clients with a sampling ratio of 0.1 and optimized for 5 local epochs. Our observations indicate that FedSOL maintains its effectiveness in both datasets, whereas FedNTD's performance decreases in CIFAR-100.

% \begingroup
% \setlength{\tabcolsep}{6.0pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1.05}
% \begin{table}[ht!]
% \small
% \vspace{-4pt}
% \caption{Test Accurac on CIFAR-100 and ImageNet-100.}
% \label{tab:cifar100_imagenet100}
% \vspace{-7pt}
% \begin{tabular}{lcccc}
% \toprule
% \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Method}}} & \multicolumn{3}{c}{\textbf{CIFAR-100}}                                           & \multicolumn{1}{c}{\textbf{ImageNet-100}} \\
%                                  & \multicolumn{1}{c}{s\,=\,5} & \multicolumn{1}{c}{s\,=\,10} & \multicolumn{1}{c}{$\alpha$\,=\,0.05} & \multicolumn{1}{c}{$\alpha$\,=\,0.1}                 \\
% \hline\hline
% FedAvg                           
% & 42.43\,\,\,                   
% & 53.23\,\,\,                      
% & 48.69\,\,\,                     
% & 43.41\,\,\,                                       \\
% FedProx                          
% & 39.03\,\footnotesize{\textcolor{red}{$\downarrow$}}                   
% & 48.38\,\footnotesize{\textcolor{red}{$\downarrow$}}                      
% & 46.75\,\footnotesize{\textcolor{red}{$\downarrow$}}                     
% & 34.49\,\footnotesize{\textcolor{red}{$\downarrow$}}                                     \\
% FedNTD                           
% & 39.32\,\footnotesize{\textcolor{red}{$\downarrow$}}                   
% & 52.23\,\footnotesize{\textcolor{red}{$\downarrow$}}                      
% & 48.35\,\footnotesize{\textcolor{red}{$\downarrow$}}                     
% & 44.08\,\footnotesize{\textcolor{green!50!black}{$\uparrow$}}                                   \\
% \hline
% \textbf{FedSOL}                    
% & \textbf{44.21}\,\footnotesize{\textcolor{green!50!black}{$\uparrow$}}                   
% & \textbf{53.78}\,\footnotesize{\textcolor{green!50!black}{$\uparrow$}}                      
% & \textbf{49.25}\,\footnotesize{\textcolor{green!50!black}{$\uparrow$}}                     
% & \textbf{44.97}\,\footnotesize{\textcolor{green!50!black}{$\uparrow$}}
% \\
% \bottomrule
% \end{tabular}
% \vspace{-12pt}
% \end{table}
% \endgroup

% \vspace{-2pt}
% \paragraph{\textcolor{orange!87!black}{fSbK}\,-\,W2 \& \textcolor{orange!87!black}{K9F1}\,-\,W1 (Computational Cost)}

% In \textbf{Table 5}, we analyze the FLOPS required for FedSOL and note that perturbing only the head part is almost as effective as full perturbation, yet it requires only 33\% more computation than FedAvg. Although FedSOL necessitates backward computation twice, this does not lead to increased GPU memory usage, as FedSOL does not store these gradients simultaneously. The slight increase in memory usage ($< 0.01$\%) arises from calculating the adaptive perturbation strength for each layer. In \autoref{tab:gpu_usage}, we present the latency for a single local step with the ImageNet-100 dataset, using a ResNet-18 model on an NVIDIA A6000 GPU. We measured FedSOL's latency using an L2 proximal loss for a fair comparison. While FedSOL involves additional local computation, we emphasize that in FL, the energy consumed for communication typically surpasses that for computation. The faster convergence of FedSOL substantially reduces the total energy consumption.
% %In the ImageNet-100 experiment detailed in \autoref{tab:cifar100_imagenet100}, for example, FedSOL achieves FedAvg's 300-round performance by round 238.
% %
% \begingroup
% \setlength{\tabcolsep}{3.0pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1.05}
% \begin{table}[ht!]
% \small
% \vspace{-4pt}
% \caption{Measured latency for a single local step.}
% \vspace{-7.5pt}
% \label{tab:gpu_usage}
% \centering
% \begin{tabular}{lccccc} 
% \toprule
% \multicolumn{1}{c}{\textbf{Usage}}     
% & \textbf{FedAvg} & \textbf{FedProx} & \textbf{FedNTD} & \textbf{FedSAM} & \textbf{FedSOL}  \\ 
% \hline\hline
% %Memory  
% %& 0000\,MB   
% %& 0000\,MB    
% %& 0000\,MB  
% %& 0000\,MB  
% %& 0000\,MB    \\
% Latency 
% & 2.846\,s    
% & 2.865\,s     
% & 2.996\,s   
% & 3.380\,s    
% & 2.900\,s     \\
% \bottomrule
% \end{tabular}
% \end{table}
% \endgroup

% \paragraph{\textcolor{orange!87!black}{fSbK}\,-\,W3 (Robustness to Communication Failure)}
% We would like to highlight that our paper includes assessments addressing \textit{communication failure}. All our experiments are based on partial client participation. For instance, in \textbf{Table 2}, we set the sampling ratio at 0.1. This indicates that only 10\% of client devices are active in each round, thereby simulating communication failures with the inactive devices. These \textit{straggler} devices might successfully communicate in subsequent rounds. The impact of the participation ratio is further assessed in \textbf{Section 4.3}. In all experiments, FedSOL consistently demonstrates performance gains, validating its robustness to communication failures.

% \vspace{-2pt}
% \paragraph{\textcolor{orange!87!black}{3HiN}\,-\,W1, W2 (Comparison to FedSAM \& FedASAM)}\,
% %
% \begin{figure}[ht!]
%     \vspace{-12pt}
%     \centering
%     \includegraphics[width=0.46\textwidth]{materials/figures/ablation_R.png}
%     \vspace{-5.5pt}
% \caption{{Performance on CIFAR-10 ($\alpha$=0.1) datasets.}}
% \label{fig:ablation_R}
% \vspace{-7pt}
% \end{figure}

% \noindent The reason we focus our comparison solely on FedAvg is to ensure clear visualization. \autoref{fig:ablation_R} presents the impact of learning factors on FedSAM and FedASAM, showing that both methods are more sensitive to these factors compared to FedSOL. Although we could not include the detailed analysis here due to the page limit, Weight Divergence is inversely related to FL performance, while Knowledge Preservation has a positive correlation with it. The related analysis will be included in the revised \textbf{Appendix}.

% \vspace{-2pt}
% \paragraph{\textcolor{orange!87!black}{3HiN}\,-\,W3 (Choice of Baselines in Table 3)} For \textbf{Table 3}, due to space constraints we selected FedAvg as the standard baseline, along with FedProx and FedNTD, which showed relatively consistent performance gains in \textbf{Table 2}. Please note that the purpose of \textbf{Table 3} is to illustrate the compatibility of FedSOL with various model architectures.

% \vspace{-2pt}
% \paragraph{\textcolor{orange!87!black}{K9F1}\,-\,W2 (Head Perturbation in Larger Models)} To address the reviewer's concerns about the effectiveness of partial perturbation strategy, we extended the comparison experiment in \textbf{Table 5} to \autoref{tab:partial_perturbation}. The results on VggNet-11 and ResNet-18 indicate that perturbing only the last classifier layer (\textit{head}) is almost as effective as perturbing the entire model (\textit{full}), saving significant computational cost.
% %
% \begingroup
% \setlength{\tabcolsep}{4.0pt} % Default value: 6pt
% \renewcommand{\arraystretch}{1.0}
% \small
% \begin{table}[ht!]
% \vspace{-1.8pt}
% \caption{Effect of partial perturbation on CIFAR-10 ($\alpha$=0.1).}
% \label{tab:partial_perturbation}
% \vspace{-7pt}
% \begin{tabular}{lccc}
% \toprule
% \multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{FedAvg}} & \multicolumn{1}{c}{\textbf{FedSOL (\textit{full})}} & \textbf{FedSOL (\textit{head})} \\
% \hline\hline
% VggNet-11
% & 41.30 
% & 56.44 \textbf{\small{\textcolor{green!60!black}{(+\,15.14)}}}  
% & 56.39 \textbf{\small{\textcolor{green!60!black}{(+\,15.09)}}} \\
% ResNet-18      
% & 49.92 
% & 66.69 \textbf{\small{\textcolor{green!60!black}{(+\,16.77)}}} 
% & 66.32 \textbf{\small{\textcolor{green!60!black}{(+\,16.04)}}}
% \\
% \bottomrule
% \end{tabular}
% \end{table}
% \endgroup
% % % References
% % {\small
% % \bibliographystyle{cvpr}
% % \bibliography{rebuttal}}
% \end{document}

==> sec/rebuttal_header.tex <==
\usepackage[rebuttal]{cvpr}

% \usepackage[sort, compress, numbers]{natbib}
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{textcomp}

\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}

% For graphics
\usepackage{graphicx}
\usepackage{mwe}
\usepackage{wrapfig}

% For algorithms
\usepackage{algorithmic}
\usepackage{algorithm}
\usepackage{tikz}
\usetikzlibrary{fit,calc}

% For tables
\usepackage{tabularx}
\usepackage{tabulary}
\usepackage{booktabs}
\usepackage{multirow}
% \usepackage{multicol}
\usepackage{arydshln}

% For Theorems
\newtheorem{theorem}{Theorem}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}

% Others
\usepackage{lipsum}
\usepackage{url}
\usepackage{blindtext}
\newenvironment{proof}{\paragraph{Proof:}}{\hfill$\square$}

% Newcommands for mathematical notation
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bwl}{\boldsymbol{w}_l}
\newcommand{\bwk}{\boldsymbol{w}_k}
\newcommand{\bwlk}{\boldsymbol{w}^k_l}
\newcommand{\bwg}{\boldsymbol{w}_g}
\makeatletter
\def\zzunderbrace#1#2{\mathop{\vtop{\m@th\ialign{##\crcr
   $\hfil\displaystyle{#1}\hfil$\crcr
   \noalign{\kern3\p@\nointerlineskip}%
   \zzupbracefill{#2}\crcr\noalign{\kern3\p@}}}}\limits}

\def\zzupbracefill#1{$\m@th \setbox\z@\hbox{$\braceld$}%
  \bracelu\leaders\vrule \@height\ht\z@ \@depth\z@\hfill
  \,\lower .1em\hbox{\scriptsize#1}\,%
  \leaders\vrule \@height\ht\z@ \@depth\z@\hfill\braceru$}
\makeatletter

% New commands for Autoref
\newcommand{\Autoref}[1]{%
  \begingroup%
  \def\algorithmautorefname{Algorithm}%
  \def\chapterautorefname{Chapter}%
  \def\sectionautorefname{Section}%
  \def\subsectionautorefname{Section}%
  \autoref{#1}%
  \endgroup%
}
\newcommand{\Tableautoref}[1]{%
  \begingroup%
  \def\figureautorefname{Table}%
  \autoref{#1}%
  \endgroup%
}

\definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
\usepackage[pagebackref,breaklinks,colorlinks,citecolor=cvprblue]{hyperref}

% Support for easy cross-referencing
\usepackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\Crefname{table}{Table}{Tables}
\crefname{table}{Tab.}{Tabs.}

\def\paperID{1898}
\def\confName{CVPR}
\def\confYear{2024}

\renewcommand{\thefigure}{R\arabic{figure}}
\renewcommand{\thetable}{R\arabic{table}}
